Explicit Non-Abelian Gerbes with Connections

We define the notion of adjustment for strict Lie 2-groups and provide the complete cocycle description for non-Abelian gerbes with connections whose structure 2-group is an adjusted 2-group. Most importantly, we depart from the common fake-flat connections and employ adjusted connections. This is an important generalisation that is needed for physical applications especially in the context of supergravity. We give a number of explicit examples; in particular, we lift the spin structure on $S^4$, corresponding to an instanton-anti-instanton pair, to a string structure, a 2-group bundle with connection. We also outline how categorified forms of Bogomolny monopoles known as self-dual strings can be obtained via a Penrose-Ward transform of string bundles over twistor space.

==> lib/characters.tex <==
\newcommand{\makecommand}[3]{%
	\foreach \i in #3 {%
    	\expandafter\xdef\csname #1\i\endcsname{{\noexpand#2{\unexpanded\expandafter{\i}}}}%
  	}%
}

%
% Characters
%

\newcommand{\latinalphabet}{A,a,B,b,C,c,d,D,E,e,F,f,G,g,H,h,I,i,J,j,K,k,L,l,M,m,N,n,O,o,P,p,Q,q,R,r,S,s,T,t,U,u,V,v,W,w,X,x,Y,y,Z,z}
\newcommand{\Latinalphabet}{A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z}

\makecommand{I}{\mathbbm}{\Latinalphabet}
\makecommand{bf}{\mathbf}{\latinalphabet}
\makecommand{bm}{\bm}{\latinalphabet}
\makecommand{ca}{\mathcal}{\Latinalphabet}
\makecommand{fr}{\mathfrak}{\latinalphabet}
\makecommand{rm}{\mathrm}{\latinalphabet}
\makecommand{sf}{\mathsf}{\latinalphabet}
\makecommand{sc}{\mathscr}{\latinalphabet}
\makecommand{tt}{\mathtt}{\latinalphabet}

\makecommand{bar}{\bar}{\latinalphabet}
\makecommand{dot}{\dot}{\latinalphabet}

\newcommand{\eps}{\varepsilon}

%
% Lie groups and algebras
%

\makecommand{sf}{\mathsf}{{GL,SL,O,SO,OSp,U,SU,Sp,Spin,String}}
\makecommand{fr}{\mathfrak}{{gl,sl,o,so,osp,u,su,sp,spin,string}}

%
% Categories etc.
%

\makecommand{Cat}{\mathsf}{{Ass,Cat,Com,DiffCat,Fun,Gr,Grp,Lie,Mfd,poSet,Set,SMfd,sGrp,sMfd,sSet,sSMfd,SurSub,Top,VectBun}}

\makecommand{sf}{\mathsf}{{CE,Ch,Diag,End,Hom,hom,hol,inthom,Jet,Kan,Lie,Ob,Map,Mat,TDiff}}


==> lib/commands.tex <==
%
% Arrows
%

\newcommand{\multirightarrow}[1]{%
	\mathrel{%
		\substack{%
			\let\multiarrowcontent\empty
			\foreach \i in {1,...,#1} {
	    		\ifnum\i=#1
	    			\expandafter\gappto\expandafter\multiarrowcontent\expandafter{\longrightarrow}
	    		\else
	    			\expandafter\gappto\expandafter\multiarrowcontent\expandafter{\longrightarrow\\[-0.6ex]}
	    		\fi
			} 
			\multiarrowcontent%
		}%
	}%
}

\newcommand{\multileftarrow}[1]{%
	\mathrel{%
		\substack{%
			\let\multiarrowcontent\empty
			\foreach \i in {1,...,#1} {
	    		\ifnum\i=#1
	    			\expandafter\gappto\expandafter\multiarrowcontent\expandafter{\longleftarrow}
	    		\else
	    			\expandafter\gappto\expandafter\multiarrowcontent\expandafter{\longleftarrow\\[-0.6ex]}
	    		\fi
			} 
			\multiarrowcontent%
		}%
	}%
}

\renewcommand{\twoheadrightarrow}{\mathrel{\mathrlap{\rightarrow}\mkern.5mu\rightarrow}}
\DeclareRobustCommand\longtwoheadrightarrow{\relbar\joinrel\twoheadrightarrow}
\renewcommand{\twoheadleftarrow}{\mathrel{\mathrlap{\leftarrow}\mkern.5mu\leftarrow}}
\DeclareRobustCommand\longtwoheadleftarrow{\twoheadleftarrow\joinrel\relbar}

%
% Derivatives
%

\newcommand{\dder}[2][]{%
	\ifthenelse{\equal{#1}{}}{%
		\frac{\mathrm{d}}{\mathrm{d} #2}%
	}{%
		\frac{\mathrm{d} #1}{\mathrm{d} #2}%
	}%
}
\newcommand{\parder}[2][]{%
	\ifthenelse{\equal{#1}{}}{%
		\frac{\partial}{\partial #2}%
	}{%
		\frac{\partial #1}{\partial #2}%
	}%
}
\newcommand{\delder}[2][]{%
	\ifthenelse{\equal{#1}{}}{%
		\frac{\delta}{\delta #2}%
	}{%
		\frac{\delta #1}{\delta #2}%
	}%
}

%
% Inner products
%

\newcommand{\inner}[2]{\langle#1,#2\rangle}
\newcommand{\innerLarge}[2]{\left\langle#1,#2\right\rangle}

%
% Vectors
%

\newcommand{\colvec}[1]{%
    \begingroup
        \newcommand\listcontent{}
        \def\do##1{\appto\listcontent{##1\\}}
        \expandafter\docsvlist\expandafter{#1}
        \begin{pmatrix}
            \listcontent
        \end{pmatrix}
    \endgroup
}

%
% Integrals
%

\DeclareMathOperator*{\sumint}{%
\mathchoice%
	{\ooalign{$\displaystyle\sum$\cr\hidewidth$\displaystyle\int$\hidewidth\cr}}
	{\ooalign{\raisebox{.14\height}{\scalebox{.7}{$\textstyle\sum$}}\cr\hidewidth$\textstyle\int$\hidewidth\cr}}
	{\ooalign{\raisebox{.2\height}{\scalebox{.6}{$\scriptstyle\sum$}}\cr$\scriptstyle\int$\cr}}
	{\ooalign{\raisebox{.2\height}{\scalebox{.6}{$\scriptstyle\sum$}}\cr$\scriptstyle\int$\cr}}
}

\newcommand{\cpv}{\setbox0=\hbox{$\int$}\int\hskip-\wd0{}\hskip-\wd0{~-~}} % Cauchy principal value

%
% Miscellaneous
%

\newcommand{\acton}{\vartriangleright} % action
\newcommand{\Ad}{\mathrm{Ad}} % adjoint map
\newcommand{\ad}{\mathrm{ad}} % adjoint map
\newcommand{\diag}{\mathrm{diag}} % diagonal matrix
\newcommand{\lvac}{\langle 0|} % vacuum
\newcommand{\dual}{^\vee} % vector space dual
\newcommand{\id}{\mathrm{id}} % identity
\newcommand{\sfid}{\mathsf{id}} % identity
\newcommand{\im}{\mathrm{im}} % image
\renewcommand{\Im}{\mathfrak{Im}} % imaginary part
\newcommand{\pr}{\mathsf{pr}} % projection
\renewcommand{\Re}{\mathfrak{Re}} % real part
\newcommand{\spacer}[1]{\vrule width0pt height0pt depth#1\relax}
\newcommand{\spn}{\mathrm{span}} % span
\newcommand{\str}{\mathrm{str}} % super trace
\newcommand{\T}{^{\mathrm{T}}} % transpose
\newcommand{\tocut}[1]{{\color{green} #1 }}
\newcommand{\todo}[1]{{\color{red} #1 }}
\newcommand{\tr}{\mathrm{tr}} % trace
\newcommand{\rvac}{|0\rangle} % vacuum
\newcommand{\uline}[1]{\ul{\emph{#1}}}
\newcommand{\unit}{\mathbbm{1}} % unit matrix
\newcommand{\rint}{\mathrm{int}}
\newcommand{\rtree}{\mathrm{tree}}
\newcommand{\lap}{\Delta}
\newcommand{\wave}{\mathop\Box}
\newcommand{\intprod}{\mathbin{\raisebox{\depth}{\scalebox{1}[-1]{$\lnot$}}}} % interior product

%
% Prepositions
%

\newcommand{\efor}{{~~~\mbox{for}~~~}}
\newcommand{\eforall}{{~~~\mbox{for all}~~~}}
\newcommand{\eand}{{~~~\mbox{and}~~~}}
\newcommand{\eon}{{~~\mbox{on}~~}}
\newcommand{\eor}{{~~~\mbox{or}~~~}}  		
\newcommand{\ewith}{{~~~\mbox{with}~~~}}

%
% Young diagrams
%

\newcommand{\tyng}[1]{\hbox{\tiny$\yng #1$}} % small Young diagram
\newcommand{\tyoung}[1]{\hbox{\tiny$\young #1$}} % small Young diagram

==> lib/hyphenation.tex <==
\hyphenation{mani-folds mani-fold opera-tor bet-ween}
